Achieving both High Energy Efficiency and High Performance in On-Chip Communication using Hierarchical Rings with Deflection Routing

Hierarchical ring networks, which hierarchically connect multiple levels of rings, have been proposed in the past to improve the scalability of ring interconnects, but past hierarchical ring designs sacrifice some of the key benefits of rings by introducing more complex in-ring buffering and buffered flow control. Our goal in this paper is to design a new hierarchical ring interconnect that can maintain most of the simplicity of traditional ring designs (no in-ring buffering or buffered flow control) while achieving high scalability as more complex buffered hierarchical ring designs. Our design, called HiRD (Hierarchical Rings with Deflection), includes features that allow us to mostly maintain the simplicity of traditional simple ring topologies while providing higher energy efficiency and scalability. First, HiRD does not have any buffering or buffered flow control within individual rings, and requires only a small amount of buffering between the ring hierarchy levels. When inter-ring buffers are full, our design simply deflects flits so that they circle the ring and try again, which eliminates the need for in-ring buffering. Second, we introduce two simple mechanisms that provides an end-to-end delivery guarantee within the entire network without impacting the critical path or latency of the vast majority of network traffic. HiRD attains equal or better performance at better energy efficiency than multiple versions of both a previous hierarchical ring design and a traditional single ring design. We also analyze our design's characteristics and injection and delivery guarantees. We conclude that HiRD can be a compelling design point that allows higher energy efficiency and scalability while retaining the simplicity and appeal of conventional ring-based designs.

==> secs/evaluation.tex <==
\section{Evaluation}
\label{sec:evaluation}

We provide an evaluation of our proposed mechanism against
other ring baselines. Since our goal is to provide a better ring design, our
main comparisons are to ring networks. We have many additional results and analyses, which
we cannot present due to space limitations. These are provided in our technical
report~\cite{hird-safari-tr}. Some of these results show our mechanism works
well with multithreaded workloads and provides better worst-case latencies than
the baselines. Additional results also provide sensitivity analyses with
different system and design parameters. See~\cite{hird-safari-tr} for details.

\subsection{Ring-based Network Designs}
\label{sec:eval-hrings}



%\noindent\textbf{Multiprogrammed workloads}


Figure~\ref{fig:hird-buf-hring} shows performance (weighted speedup
normalized per node), power (total network power normalized per node),
and energy-efficiency (perf./power) for 16-node and 64-node HiRD and
buffered hierarchical rings in~\cite{ravindran97}, using identical topologies, as well as a
single ring (with different bisection bandwidths).
%\footnote{Since our goal
%is to provide a better ring design, our main comparisons are to ring
%networks. Section~\ref{sec:eval-topos} provides an evaluation of other
%topologies.} Several major conclusions are in order:



1. A hierarchical topology yields significant performance advantages over a
single ring (i) when network load is high and/or (ii) when the network scales
to many nodes. As shown, the buffered hierarchical ring improves
performance by 7\% (and HiRD by 10\%) %over the single ring %%GL: you say "compared to a single ring" immediately below again
in high-load workloads at 16 nodes compared to a single ring with 128-bit links. The
hierarchical design also reduces power because hop count is reduced. Therefore,
link power reduces significantly with respect to a single ring.
\ignore{
2. HiRD improves performance over the buffered hierarchical ring in larger
networks, where the scaling advantage of hierarchy becomes more important.}
On average, in the 8x8 configuration, the buffered hierarchical ring network
obtains 15.6\% better application performance than the single ring with 256-bit
links, while HiRD attains 18.2\% higher performance.

2. Compared to the buffered hierarchical ring, HiRD has significantly
lower network power and better performance. On average, HiRD reduces total network power
(links and routers) by 46.5\% (4x4) and 14.7\% (8x8) relative to this
baseline. This reduction in turn yields significantly better energy
efficiency (lower energy consumption for buffers and slightly higher for links). 
Overall, HiRD is the most energy-efficient of the
ring-based designs evaluated in this paper for both 4x4 and 8x8 network
sizes. HiRD also performs better than Buffered HRing due to the reasons explained
in the next section (\S\ref{sec:eval-synth}).

3. While scaling the link bandwidth increases the performance of a single ring
network, the network power increases 25.9\% when the link bandwidth increases
from 64-bit to 128-bit and  15.7\% when the link bandwidth increases from
128-bit to 256-bit because of higher dynamic energy due to wider links.
\ignore{Additionally, given the same amount of energy consumed by the network,
increasing link bandwidth increases the performance, which will increase the
power consumption as power is energy over time.} In addition, scaling the link
bandwidth is not a scalable solution as a single ring network performs worse
than the bufferred hierarchical ring baseline even when a 256-bit link is used.

Our technical report~\cite{hird-safari-tr} contains more analyses and
additional evaluations on several multithreaded workloads. Our results show that
HiRD is more energy-efficient than both the single ring designs and the
buffered hierarchical ring design.

\linespread{0.95}
\begin{table*}
\vspace{-0.25in}
%\begin{table*}[h!]
\small
\centering
%\vspace{-0.1in}
\begin{tabular}{|l||l|l|l||l|l|}
\hline
Configuration &  \multicolumn{3}{|c||}{\breakTable{Network Throughput\\(flits/node/cycle)}} & Transfer FIFO Wait (cycles) & Deflections/Retries \\
\hline
 & Ring A & Ring B & Ring C & avg/max & avg/max \\
\hline
\hline
Without Guarantees & 0.164 & 0.000 & 0.163 & 2.5 / 299670 & 6.0 / 49983 \\
\hline
With Guarantees & 0.133 & 0.084 & 0.121 & 1.2 / 66 & 2.8 / 18 \\
\hline
\end{tabular}
\caption{\footnotesize \bf Results of worst-case traffic pattern without and with
  injection/transfer guarantees enabled.}
\label{table:guarantee-results}
\vspace{-0.3in}
\end{table*}
\linespread{0.85}


%\linespread{0.95}
%\begin{table*}
%\vspace{-0.25in}
%%\begin{table*}[h!]
%\small
%\centering
%%\vspace{-0.1in}
%\begin{tabular}{|l||l|l||l|l|l|}
%\hline
%Configuration & Transfer FIFO Wait (cycles) & Deflections/Retries & \multicolumn{3}{|c|}{\breakTable{Network Throughput\\(flits/node/cycle)}} \\
%\hline
% & avg/max & avg/max & Ring A & Ring B & Ring C \\
%\hline
%\hline
%Without Guarantees & 2.5 / 299670 & 6.0 / 49983 & 0.164 & 0.000 & 0.163 \\
%\hline
%With Guarantees & 1.2 / 66 & 2.8 / 18 & 0.133 & 0.084 & 0.121 \\
%\hline
%\end{tabular}
%\caption{\small Results of worst-case traffic pattern without and with
%  injection/transfer guarantees enabled.}
%\label{table:guarantee-results}
%\vspace{-0.3in}
%\end{table*}
%\linespread{0.85}


%\noindent\textbf{Multithreaded workloads}
%
%\begin{figure*}
%\vspace{-0.2in}
%\centering
%\includegraphics[width=5.4in]{plots/eval_rings_graph.pdf}
%\caption{\small HiRD as compared to buffered hierarchical rings and a single-ring network.}
%\label{fig:hird-buf-hring-graph}
%\end{figure*}
%
%Figure~\ref{fig:hird-buf-hring-graph} shows the performance and power of
%multithreaded applications of HiRD compared a buffered hierarchical ring and a
%single-ring network for both 16-node and 64-node systems. On average, HiRD
%performs 0.1\% (4x4) and 0.73\% (8x8) worse than the buffered hierarchical ring.
%However, on average, HiRD consumes 43.8\% (4x4) and 3.1\% (8x8) less power,
%leading to higher energy efficiency. 
%
%Both the buffered hierarchical ring and HiRD outperform single ring networks,
%both in performance and energy efficiency, and the gap increases as we scale the
%size of the network.
%
%Even though HiRD performs competitively with a buffered hierarchical ring
%network in most cases, HiRD performs poorly on the Page Ranking application. We
%observe that Page Ranking generates more non-local network traffic. As a
%result, the advantage of HiRD where the local-ring latency is lower does not
%provide speedup for Page Ranking. In addition, Page Ranking also has higher
%network traffic, causing more congestion in the network (we observe 17.3\%
%higher average network latency for HiRD in an 8x8 network), which causes
%additional performance drop for HiRD. However, it is potentially possible to
%use a different number of bridge routers as illustrated in
%Figure~\ref{fig:topology}, to improve the performance of HiRD.  We will provide this analysis in
%Section~\ref{sec:eval-sensitivity}.  Additionally, it is possible to apply a
%locality-aware cache mapping technique~\cite{CloudCache} in order to take advantage of
%lower local-ring latency in HiRD.
%

\subsection{Synthetic-Traffic Network Behavior}
\label{sec:eval-synth}


\begin{figure}[h!]
%\vspace{-0.1in}
\centering
\subfloat[Uniform Random, 4x4]{
\includegraphics[width=1.5in]{plots/synthUR.pdf}
\label{fig:synthUR}
}
\subfloat[Uniform Random, 8x8]{
\includegraphics[width=1.5in]{plots/synth8UR-new.pdf}
\label{fig:synth8UR}
}
\\
\vspace{-0.1in}
\subfloat[Bit Complement, 4x4]{
\includegraphics[width=1.5in]{plots/synthBC.pdf}
\label{fig:synthBC}
}
\subfloat[Bit Complement, 8x8]{
\includegraphics[width=1.5in]{plots/synth8BC.pdf}
\label{fig:synth8BC}
}
\\
\vspace{-0.1in}
\subfloat[Transpose, 4x4]{
\includegraphics[width=1.5in]{plots/synthTR.pdf}
\label{fig:synthTR}
}
\subfloat[Transpose, 8x8]{
\includegraphics[width=1.5in]{plots/synth8TR.pdf}
\label{fig:synth8TR}
}
\vspace{-0.05in}
\caption{\footnotesize \bf Synthetic-traffic evaluations for 4x4 and 8x8 networks.}
\label{fig:synth}
\vspace{-0.15in}
\end{figure}


Figure~\ref{fig:synth} shows the average packet latency as a function of injection rate for
buffered and bufferless mesh routers, a single-ring design, the buffered
hierarchical ring, and HiRD in 16 and 64-node systems. We show uniform random,
transpose and bit complement traffic patterns~\cite{principles}. Sweeps on injection rate
terminate at network saturation. The buffered hierarchical ring saturates at a
similar point to HiRD but maintains a slightly lower average latency because it
avoids transfer deflections. In contrast to these high-capacity designs, the
256-bit single ring saturates at a lower injection rate. As network size scales to 8x8,
HiRD performs significantly better than the 256-bit single ring, because the
hierarchy reduces the cross-chip latency while preserving bisection bandwidth.
HiRD also performs better than Buffered HRing because of two reasons. First,
HiRD is able to allow higher peak utilization (91\%) than Buffered HRing (71\%)
on the global rings. We observed that when flits have equal distance in a
clock-wise and counter clock-wise direction, Buffered HRing has to send flits
to one direction in order to avoid deadlock while deflections in HiRD allow
flits to travel in both directions, leading to better overall network
utilization. Second, at high injection rates, the transfer guarantee
(\S\ref{sec:guarantees}) starts throttling the network, disallowing
future flits to be injected into the network until the existing flits arrive at
their destinations. This reduces congestion in the network and allows HiRD to
saturate at a higher injection rate than the buffered hierarchical ring design.


\ignore{
Figure~\ref{fig:synth} shows average latency as a function of injection rate for
buffered and bufferless mesh routers, a single-ring design, the buffered
hierarchical ring, and HiRD in 16 and 64-node systems. We show uniform random,
transpose, and bit-complement traffic patterns. Sweeps terminate at network
saturation. For comparison, we also add a buffered mesh with buffer bypassing
and CHIPPER~\cite{chipper}, a bufferless mesh network. HiRD performs very
closely to the buffered mesh design in 4x4, saturating at nearly the same
injection rate but maintaining a slightly lower network latency at high load.
The buffered hierarchical ring saturates at a similar point to HiRD and the
buffered mesh, but maintains a slightly lower average latency because it avoids
transfer deflections. In contrast to these high-capacity designs, the single
ring saturates at a lower injection rate, closer to the bufferless mesh design,
CHIPPER. As network size scales to 8x8, HiRD performs significantly better
relative to the meshes, because the hierarchy reduces the cross-chip latency
while preserving bisection bandwidth.  Lastly, HiRD also performs better than
Buffered HRing because of two reasons. First, HiRD is able to allow higher
peak utilization (91\%) than Buffered HRing (71\%) on the global rings. We
observed that when flits have equal distance in a clock-wise and counter
clock-wise direction, Buffered HRing has to send flits to one direction in
order to avoid deadlock while deflections in HiRD allow flits to travel in
both directions, leading to better overall network utilization. Second, at high injection rates, the transfer guarantee (Section~\ref{sec:guarantees}) starts
throttling the network, disallowing future flits to be injected into the network
until the existing flits arrive at their destinations. This reduces congestion
in the network and allow HiRD to saturate after a buffered 
hierarchical ring design.
}

\ignore{
\begin{figure}[h!]
\centering
%\vspace{-0.15in}
\includegraphics[width=4in]{plots/synthHRStage.pdf}
\caption{\small Uniform Random synthetic traffic sweeping the number 
of pipeline stages in a hierarchical ring 8-bridge design}
\label{fig:synthStage}
\end{figure}
}

\subsection{Injection and Transfer Guarantees}
\label{sec:eval-guarantees}


In this subsection, we study HiRD's behavior under a worst-case
synthetic traffic pattern that triggers the injection and transfer
guarantees and demonstrates that they are necessary for correct
operation, and that they work as designed.


\noindent\textbf{Traffic Pattern:} In the worst-case traffic pattern, all nodes
on three rings in a two-level (16-node) hierarchy inject traffic (we call these
rings Ring A, Ring B, and Ring C). Rings A, B, and C have bridge routers
adjacent to each other, in that order, on the single global ring. All nodes in
Ring A continuously inject flits 
%that are addressed 
to nodes in Ring C, and all
nodes in Ring C likewise inject flits to nodes in Ring A. This creates heavy
traffic on the global ring across the point at which Ring B's bridge router
connects. All nodes on Ring B continuously inject flits (whenever they are
able) addressed to another ring elsewhere in the network. However, because
Rings A and C continuously inject flits, Ring B's bridge router will not be
able to transfer any flits to the global ring in the steady state (unless
another mechanism such as the throttling mechanism in
\S\ref{sec:guarantees} intercedes).



\noindent\textbf{Results:} Table~\ref{table:guarantee-results} shows
three pertinent metrics on the network running the described traffic
pattern: average network throughput (flits/node/cycle) for nodes on
Rings A, B, and C, the maximum time (in cycles) spent by any one flit
at the head of a transfer FIFO, and the maximum number of times any
flit is deflected and has to circle a ring to try again. These metrics
are reported with the injection and transfer guarantee mechanisms
disabled and enabled. The experiment is run with the synthetic traffic
pattern for 300K cycles.

The results show that \emph{without} the injection and transfer guarantees,
Ring B is completely starved and cannot transfer any flits onto the
global ring. This is confirmed by the maximum transfer FIFO wait time,
which is almost the entire length of the simulation. In other words,
once steady state is reached, no flit ever transfers out of Ring
B. Once the transfer FIFO in Ring B's bridge router fills, the local
ring fills with more flits awaiting a transfer, and these flits are
continuously deflected. Hence, the maximum deflection count is very
high.  Without the injection or transfer guarantees, the network does
\emph{not} ensure forward progress for these flits. In contrast, when
the injection and transfer guarantees are enabled, (i) Ring B's bridge
router is able to inject flits into the global ring and (ii) Ring B's
bridge router fairly picks flits from its local ring to place into its
transfer FIFO. The maximum transfer FIFO wait time and maximum
deflection count are now bounded, and nodes on all rings receive
network throughput.  Thus, the guarantees are both necessary
and sufficient to ensure deterministic forward progress for all flits
in the network. 

Our technical report~\cite{hird-safari-tr} provides similar worst-case analyses
for real workloads as well as additional network latency results. We have shown in~\cite{hird-safari-tr}
that the injection and transfer guarantees also lower network latency while
deflections help to balance network load under heavy traffic.

%\begin{table}
%\small
%\centering
%\vspace{-0.2in}
%\begin{tabular}{|l||l|l|}
%\hline
%Configuration & Transfer FIFO Wait & Deflections/Retries \\
%\hline
% & (avg/max) & (avg/max) \\
%\hline
%\hline
%Without guarantees & 3.3 / 169 & 3.7 / 19 \\
%\hline
%With guarantees & 0.76 / 72 & 0.7 / 8 \\
%\hline
%\end{tabular}
%\caption{\small Effect from transfer guarantee mechanism on real workloads.}
%\label{table:guarantee-real-results}
%%\vspace{-0.1in}
%\end{table}
%
%\noindent\textbf{Real Applications:} Table~\ref{table:guarantee-real-results}
%shows the effect of the transfer guarantee mechanism on real applications in a
%4x4 network.  Average transfer FIFO wait shows the average number of cycles
%that a flit waits on average in the transfer FIFO across all 60 workloads.
%Maximum transfer FIFO wait shows the maximum observed latency across all
%workloads.  As illustrated in Table~\ref{table:guarantee-real-results}, a few
%flits can experience very high wait time when there is no transfer guarantee,
%and our transfer guarantee mechanism reduces both average and maximum FIFO
%waits\footnote{As the network scales to 64 nodes, we observe that the average
%wait in the transfer FIFO does not affect the overall performance significantly
%(additional 1.5 cycles per flit).}. In addition, we observe that our transfer
%guarantee mechanism not only provides livelock- and deadlock-freedom but also
%provides lower maximum wait time in the transfer FIFO for each flit because
%the guarantee provides a form of throttling when the network is congested. This
%similar observation is also discussed in many previous network-on-chip works
%that use source throttling to improve the performance of the
%network~\cite{selftuned,baydal05,hotnets2010,hat-sbac-pad}.

%\subsection{Network Latency and Latency Distribution}
%
%\begin{figure*}
%%\begin{figure*}[h!]
%\centering
%%\vspace{-.2in}
%\includegraphics[width=5in]{plots/avgLatency.pdf}
%%\vspace{-.2in}
%\caption{Average network latency for 4x4 and 8x8 networks.}
%%\vspace{-.1in}
%\label{fig:avg_Latency}
%\end{figure*}
%
%Figure~\ref{fig:avg_Latency} shows average network latency. This plot
%shows that our proposal can reduce the network latency by having a faster
%local-ring hop latency compared to other ring-based designs. Additionally,
%we found that, for all real workloads, the number of deflections we
%observed is always less than 3\% of the total number of flits. Therefore,
%the benefit of our deflection based router design outweighs the extra cost
%of deflections compared to other ring-based router designs.
%
%\begin{figure*}
%%\begin{figure*}[h!]
%\centering
%%\vspace{-.2in}
%\includegraphics[width=5in]{plots/maxLatency.pdf}
%%\vspace{-.2in}
%\caption{Maximum network latency for 4x4 and 8x8 networks.}
%\vspace{-.1in}
%\label{fig:max_Latency}
%\end{figure*}
%
%\begin{figure*}
%%\begin{figure*}[h!]
%\centering
%\vspace{-.1in}
%\includegraphics[width=5in]{plots/95thLatency.pdf}
%%\vspace{-.2in}
%\caption{95th percentile latency for 4x4 and 8x8 networks.}
%%\vspace{-.1in}
%\label{fig:95th_Latency}
%\end{figure*}
%
%In addition, Figure~\ref{fig:max_Latency} shows the maximum latency 
%and Figure~\ref{fig:95th_Latency} shows the 95th percentile
%latency for each network design. These two figures provide a quantitative evidence
%that the network is deadlock-free and livelock-free. Several additional
%observations are in order:
%
%1. HiRD provides lower latency at the 95th percentile and the lowest
%latency observed in the network. This lower latency comes from our transfer
%guarantee mechanism that is applied when flits spend more than 100 cycles in
%each local ring, draining all flits in the network to their destination. This
%also means that HiRD improves the worst case latency that a flit can
%experience because none of the flits are severely slowed down.
%
%2. While both HiRD and the buffered hierarchical ring have higher 95th percentile
%and maximum flit latency compared to a 64-bit single ring network, both hierarchical
%designs have 60.1\% (buffered hierarchical ring) and 53.9\% (HiRD) lower
%average network latency in an 8x8 network because hierarchy provides better scalability on average. 
%
%3. Maximum latency in the single ring is low because contention happens only at
%injection and ejection, as opposed to hierarchical designs where contention can
%also happen when flits travel through different hierarchies.
%
%4. The transfer guarantee in HiRD also helps to significantly reduce the maximum
%latency observed by some flits compared to a buffered design because the
%guarantee enables the throttling of the network, thereby alleviating congestion.
%Reduced congestion leads to reduced maximum latency. This observation is confirmed with our synthetic
%traffic results shown in Section~\ref{sec:eval-synth}
%
\subsection{Router Area and Timing}
\label{sec:eval-area}

We show both critical path length and normalized die area for single-ring,
buffered hierarchical ring, and HiRD, in Table~\ref{table:timing_area}. Area
results are normalized to the buffered hierarchical ring baseline, and are
reported for all routers required by a 16-node network (e.g., for HiRD, 16 node
routers and 8 bridge routers).

%\begin{table}
\linespread{1}
\begin{table}[h!]
\centering
\vspace{-0.1in}
\footnotesize{
\begin{tabular}{|p{1.9cm}||p{15mm}|p{20mm}|p{10mm}|}
\hline
Metric & Single-Ring & Buffered HRing & HiRD \\
\hline
\hline
Critical path (ns) & 0.33 & 0.87 & 0.61 \\
%Critical path length (ns) & 0.33 & 0.87 & 0.61 \\
\hline
Normalized area & 0.281 & 1 & 0.497 \\
\hline
\end{tabular}
}
\vspace{-0.05in}
\caption{\footnotesize \bf Total router area (16-node network) and critical path.}
\label{table:timing_area}
%\vspace{-0.25in}
\vspace{-0.15in}
\end{table}

\linespread{0.85}


Two observations are in order. First, HiRD reduces area relative to the
buffered hierarchical ring routers, because the node router required at each
network node is much simpler and does not require complex flow control logic.
HiRD reduces total router area by 50.3\% vs. the buffered hierarchical ring.
Its area is higher than a single ring router because it contains buffers in
bridge routers. However, the energy efficiency of HiRD and its performance at
high load make up for this shortcoming. Second, the buffered
hierarchical ring router's critical path is 42.6\% longer than HiRD because its control
logic must also handle flow control (it must check whether credits are
available for a downstream buffer).  The single-ring network has a higher
operating frequency than HiRD because it does not need to accommodate ring
transfers (but recall that this simplicity comes at the cost of poor
performance at high load for the single ring).

\ignore{
We show both critical path length and normalized die area for buffered and
bufferless mesh, single-ring, buffered hierarchical ring, and HiRD, in
Table~\ref{table:timing_area}. Area results are normalized by the buffered mesh
baseline, and are reported for all routers required by a 16-node network (e.g.,
for HiRD, 16 node routers and 8 bridge routers). 
%\footnote{In order to see the worst case scenario in case the critical
%path of HiRD is worse than a buffered hierarchical ring router, we perform an
%experiment where we add one extra cycle router latency for HiRD to reflect the
%worst case critical path. In this case, the HiRD performs 3.65\% worse than
%buffered hierarchical ring}. 

Two observations are in order. First, hierarchical ring designs in
general significantly reduce area relative to the buffered hierarchical ring routers,
because the node router required at each network node is much simpler
and does not require complex flow control logic. HiRD
reduces total router area by 50.3\% vs. the buffered mesh. Its area
is higher than a single ring router because it contains
buffers in bridge routers. However, the energy efficiency of HiRD
and its performance at high load make up for this shortcoming. Second,
unlike HiRD's, the buffered hierarchical ring router's critical path is 42.6\%
longer  because its control logic must also handle flow control (it must check
whether credits are available for a downstream buffer).
The single-ring network has a higher operating frequency than HiRD
because it does not need to accommodate ring transfers (but recall
that this simplicity comes at the cost of poor performance at high
load for the single ring).
}


\ignore{
\begin{table}[h!]
\centering
\footnotesize{
\begin{tabular}{|p{1.5cm}||p{8mm}|p{10mm}|p{7mm}|p{8mm}|p{7mm}|}
\hline
Metric & Buffered & CHIPPER & Single-Ring & Buffered HRing & HiRD \\
\hline
\hline
Critical path length (ns) & 1.21 & 0.93 & 0.33 & -- & 0.61 \\
\hline
Normalized area & 1 & 0.181 & 0.205 & 0.729 & 0.362 \\
\hline
\end{tabular}
}
\caption{\footnotesize \bf Total router area (16-node network) and critical path.}
\label{table:timing_area}
\vspace{-0.3in}
\end{table}
}

%\subsection{Sensitivity Studies}
%\label{sec:eval-sensitivity}
%
%\subsubsection{Sensitivity to Link Bandwidth}
%
%\begin{figure*}
%%\begin{figure*}[h!]
%\centering
%%\vspace{-.2in}
%\includegraphics[width=5in]{plots/bw_main.pdf}
%%\vspace{-.2in}
%\caption{Sensitivity to different link bandwidth for 4x4 and 8x8 networks.}
%%\vspace{-.1in}
%\label{fig:bw_sweep}
%\end{figure*}
%
%The bandwidth of each link also has an effect on the performance of different
%network designs. In this subsection, we evaluate the effect of different link
%bandwidths on several ring-based networks by using 32- 64- and 128-bit links on all
%network designs. Figure~\ref{fig:bw_sweep} shows the performance and power
%consumption of each network design. As links get
%wider, the performance of each design increases.  According to the result, HiRD performs
%slightly better than a buffered hierarchical ring design for almost all link
%bandwidths while maintaining much lower power consumption on a 4x4 network, and
%slightly lower power consumption on an 8x8 network. 
%
%Additionally, we observe that increasing link bandwidth can decrease the network
%power in a hierarchical design because lower link bandwidth causes more
%congestion in the network and leads to more dynamic buffer, crossbar and link power
%consumption due to additional deflections at the buffers. 
%As the link bandwidth increases, congestion reduces, lowering
%dynamic power. However, we observe that past a certain link bandwidth (e.g., 128 bits for
%buffered hierarchical ring and HiRD), congestion no longer reduces, because
%deflections at the buffers become the bottleneck instead. This leads to
%diminishing returns in performance yet increased dynamic power.
%\ignore{We also observe that this behavior saturates once the link
%bandwidth in large enough (128-bit for buffered hierarchical ring and HiRD),
%leading to no further performance gain and increased dynamic power because
%links that are too large do not reduce the overall deflections
%at the buffer any further. 
%In this scenario, we observe that more energy is
%required to transfer a packet to the destination, but the time a packet takes 
%to reach its destination (packet latency) decreases. As power is energy over time,
%wide links lead to higher average power consumption.}
%
%\subsubsection{Sensitivity to Configuration Parameters}
%
%\noindent\textbf{Bridge Router Organization:} The number of bridge
%routers that connect the global ring(s) to the local rings has an
%important effect on system performance because the connection between
%local and global rings can limit bisection bandwidth. In
%Figure~\ref{fig:topology}, we showed three alternative arrangements for
%a 16-node network, with 4, 8, and 16 bridge routers. So far, we have
%assumed an 8-bridge design in 4x4-node systems, and a system with 8
%bridge routers at each level in 8x8-node networks
%(Figure~\ref{fig:scale}). In Figure~\ref{fig:bridges}, we show average
%performance across all workloads for a 4x4-node system with 4, 8, and
%16 bridge routers. Buffer capacity is held constant. As shown,
%significant performance is lost if only 4 bridge routers are used
%(10.4\% on average). However, doubling from 8 to 16 bridge routers
%gains only 1.4\% performance on average. Thus, the 8-bridge design
%provides the best tradeoff of performance and network cost (power and
%area) overall in our evaluations.
%
%\begin{figure*}
%%\begin{figure*}[h!]
%\centering
%%\vspace{-0.4in}
%%\hspace{-1.4in}
%\subfloat[\scriptsize Number of bridge routers]{
%\includegraphics[width=1.25in]{plots/bridges.pdf}
%\label{fig:bridges}
%}
%%\hspace{1in}
%\subfloat[\scriptsize Local-to-global bridge buffer]{
%\includegraphics[width=1.25in]{plots/L2GBuf.pdf}
%\label{fig:L2GBuf}
%}
%%\\
%\subfloat[\scriptsize Global-to-local bridge buffer]{
%\includegraphics[width=1.25in]{plots/G2LBuf.pdf}
%\label{fig:G2LBuf}
%}
%%\hspace{1in}
%\subfloat[\scriptsize Global-Local ring B/W ratio]{
%\includegraphics[width=1.25in]{plots/GWidth.pdf}
%\label{fig:GWidth}
%}
%\caption{\small Performance sensitivity to buffer sizes and the global ring
%  bandwidth in a 4x4 network.}
%\end{figure*}
%
%
%
%\noindent\textbf{Bridge Router Buffer Size:} The size of the FIFO
%queues that are used to transfer flits between local and global rings
%can have an impact on performance if they are too small (and hence are
%often full and deflect transferring flits) or too large (and hence
%increase bridge router power and die area). We show the effect of
%local-to-global and global-to-local FIFO sizes in
%Figs.~\ref{fig:L2GBuf}~and~\ref{fig:G2LBuf}, respectively, for the
%8-bridge 4x4-node design. In both cases, increased buffer size leads
%to increased performance. However, performance is more sensitive to
%global-to-local buffer size (20.7\% gain from 1 to 16-flit buffer
%size) than local-to-global size (10.7\% performance gain from 1 to 16
%flits), because in the 8-bridge configuration, the whole-loop latency
%around the global ring is slightly higher than in the local rings, so
%a global-to-local transfer retry is more expensive.
%% 4.9% less power from 1 to 16 global-to-local; 0.9% more power from 1 to 16 local-to-global
%For our evaluations, we use a 4-flit global-to-local and 1-flit
%local-to-global buffer per bridge router, which results in transfer
%deflection rates of 28.2\% (global-to-local) and 34\%
%(local-to-global).\ignore{The system designer can tune
%  these parameters to optimize for power or performance as desired.}
%
%
%\noindent\textbf{Global Ring Bandwidth:} Previous work on
%hierarchical-ring designs did not examine the impact of global-ring
%bandwidth on performance, but instead, assumed equal bandwidth in
%local and global rings~\cite{ravindran98}. In Figure~\ref{fig:GWidth},
%we examine the sensitivity of system performance to global ring
%bandwidth relative to local ring bandwidth, for the all-High category
%of workloads (in order to stress bisection bandwidth). Each point in
%the plot is described by this bandwidth ratio. The local ring design
%is held constant while the width of the global ring is adjusted. If a
%ratio of 1:1 is assumed (leftmost bar), performance is significantly
%worse than the best possible design. Our main evaluations in 4x4
%networks use a ratio of 2:1 (global:local) in order to provide
%equivalent bisection bandwidth to a 4x4 mesh baseline. Performance
%increases by 81.3\% from a 1:1 ratio to the 2:1 ratio that we
%use. After a certain point, the global ring is no longer the
%bottleneck, and further global-ring bandwidth increases have little
%effect. \ignore{Nevertheless, a high-ratio design point might be
%  desirable to ameliorate concerns of worst-case performance under
%  very high network load, at the cost of additional global ring area
%  and energy.}
%
%\noindent\textbf{Delivery guarantee parameters:} In
%Section~\ref{sec:livelock}, we introduced injection guarantee and ejection
%guarantee mechanisms to ensure every flit is eventually delivered. The
%injection guarantee mechanism takes a threshold parameter that
%specifies how long an injection can be blocked before action is taken.
%Setting this parameter too low can have an adverse impact on
%performance, because the system throttles too aggressively and thus
%underutilizes the network. Our main evaluations use a $100$-cycle
%threshold. For High-intensity workloads, performance drops 21.3\% when
%using a threshold of only $1$ cycle. From $10$ cycles upward,
%variation in performance is at most 0.6\%: the mechanism is invoked
%rarely enough that the exact threshold does not matter, only that it
%is finite (for correctness). In fact, for a 100-cycle threshold, the
%injection guarantee mechanism is never triggered in our realistic
%workloads. The mechanism is necessary only for corner-case
%correctness. In addition, we evaluate the impact of communication
%latency between routers and the coordinator. We find less than 0.1\%
%variation in performance for latencies from $1$ to $30$ cycles (when
%parameters are set so that the mechanism becomes active); thus,
%low-cost, slow wires may be used for this mechanism.
%
%The ejection guarantee takes a single threshold parameter: the number
%of times a flit is allowed to circle around a ring before action is
%taken. We find less than 0.4\% variation in performance with a
%threshold from $1$ to $16$.  Thus, the mechanism provides correctness
%in corner cases but is unimportant for performance in the common case.
%

%TODO: Check
%\ignore{
\subsection{Comparison Against Other Ring Configurations}
\label{sec:eval-ws-power}

Figure~\ref{fig:WS_power} highlights the energy-efficiency comparison of
different ring-based design configurations by showing weighted speedup (Y axis)
against power (X axis) for all evaluated 4x4 networks. HiRD is shown with the
three different bridge-router configurations (described in
\S\ref{sec:bridge_router}). Every ring design is evaluated at various
link bandwidths (32-, 64-, 128- and 256-bit links). The top-left is the ideal
corner (high performance, low power). As the results show, at the same link
bandwidth, all three configurations of HiRD are more energy efficient than the
evaluated buffered hierarchical ring baseline designs at this network size.

\begin{figure}[h!]
\vspace{-.35in}
\centering
\hbox{
\hspace{-.35in}
\includegraphics[width=3.85in]{plots/WS_power_excel.pdf}
}
\vspace{-.3in}
\caption{\footnotesize \bf Weighted speedup (Y) vs. power (X) for 4x4 networks.}
\vspace{-.15in}
\label{fig:WS_power}
\end{figure}



We also observe that increasing link bandwidth can sometimes decrease router
power as it reduces deflections in HiRD or lowers contention at the buffers in
a buffered hierarchical ring design. However, once links are wide enough, this
benefit diminishes for two reasons: 1) 
%discussed in Section~\ref{sec:eval-sensitivity} (
links and crossbars consume more energy, 2)
packets arrive at the destination faster, leading to higher power as more energy
is consumed in less time.
%}

Aside from the comparison against other ring configurations, comparisons
against other network topologies such as buffered~\cite{dally-vc} and
bufferless~\cite{chipper} meshes and flattened butterfly~\cite{flattened_bfly},
are available in our technical report~\cite{hird-safari-tr}. We show
in~\cite{hird-safari-tr} that HiRD is more energy efficient than these network
topologies.

\ignore{Additionally, we provide two additional comparison points against two flattened
butterfly designs. First, compared to the flatten butterfly design that has
equal bisection bandwidth (FbFly Eq. BW), HiRD performs 8.14\% better and also
consumes 53\% less power. Compared to the 64-bit link flatten butterfly, HiRD
performs 2.69\% slower, but consumes 58\% less power. }

%\subsection{Comparison Against Other Network Designs}
%\label{sec:eval-topos}
%
%For completeness, Table~\ref{table:results-topo} shows the comparison against several other network
%designs on 4x4 and 8x8 networks using the multiprogrammed workloads described in
%Section~\ref{sec:meth}.
%
%
%\ignore{
%For completeness, Figure~\ref{fig:synth-topo} shows the comparison against several other network
%designs on a 4x4 and 8x8 network using a synthetic workloads similar to
%Section~\ref{sec:eval-synth}.
%
%\begin{figure}[h!]
%\centering
%\subfloat[Uniform Random, 4x4]{
%\includegraphics[width=1.75in]{plots/synthUR_topo.pdf}
%\label{fig:synthUR-topo}
%}
%\subfloat[Bit Complement, 4x4]{
%\includegraphics[width=1.75in]{plots/synthBC_topo.pdf}
%\label{fig:synthBC-topo}
%}
%\subfloat[Transpose, 4x4]{
%\includegraphics[width=1.75in]{plots/synthTR_topo.pdf}
%\label{fig:synthTR-topo}
%}
%\\
%\subfloat[Uniform Random, 8x8]{
%\includegraphics[width=1.75in]{plots/synth8UR_topo.pdf}
%\label{fig:synth8UR-topo}
%}
%\subfloat[Bit Complement, 8x8]{
%\includegraphics[width=1.75in]{plots/synth8BC_topo.pdf}
%\label{fig:synth8BC-topo}
%}
%\subfloat[Transpose, 8x8]{
%\includegraphics[width=1.75in]{plots/synth8TR_topo.pdf}
%\label{fig:synth8TR-topo}
%}
%\caption{\small Synthetic-traffic evaluations for 4x4 and 8x8 networks against different topologies.}
%\label{fig:synth-topo}
%\end{figure}
%}
%
%We compared our mechanism against a buffered mesh design with buffer bypassing.
%We configure the buffered mesh to have 4 VCs per port with 8 buffers per VC.
%We also compare our mechanism against CHIPPER~\cite{chipper}, a bufferless mesh
%network. We use 128-bit links for both designs.  Additionally, we compare our
%mechanism against a flattened butterfly~\cite{flattened_bfly}
%with 4 VCs per output port, 8 buffers per VC and 64-bit links. Our conclusions
%are as follows:
%
%\begin{table*}
%\small
%\centering
%%\vspace{-0.2in}
%\begin{tabular}{|l||l|l||l|l|}
%\hline
%Topologies & \multicolumn{2}{c||}{4x4} & \multicolumn{2}{|c|}{8x8} \\
%\hline
% & Norm. WS & Power (mWatts) & Norm. WS & Power (mWatts) \\
%\hline
%\hline
%Single Ring & 0.904 & 7.696 & 0.782 & 13.603 \\
%\hline
%Buffered HRing & 1 & 12.433 & 1 & 16.188 \\
%\hline
%Buffered Mesh & 1.025 & 11.947 & 1.091 & 13.454 \\
%\hline
%CHIPPER & 0.986 & 4.631 & 1.013 & 7.275 \\
%\hline
%Flattened Butterfly & 1.037 & 10.760 & 1.211 & 30.434 \\
%\hline
%HiRD & 1.020 & 4.746 & 1.066 & 12.480 \\
%\hline
%\end{tabular}
%\caption{\small Evaluation for 4x4 and 8x8 networks against different network designs}
%\label{table:results-topo}
%%\vspace{-0.1in}
%\end{table*}
%
%
%
%%TODO: rewrite this
%%\footnote{flattened butterfly
%%design has higher bisection bandwidth compared to other designs.}. 
%
%1. Compared to designs using the mesh topology, we observe that HiRD performs very
%closely to the buffered mesh design both for 4x4 and 8x8 network sizes while a
%buffered hierarchical ring design performs slightly worse compared to HiRD and
%buffered mesh designs. Additionally, HiRD performs better than CHIPPER in both
%4x4 and 8x8 networks but CHIPPER consumes less power in an 8x8 design as there
%is no buffer in CHIPPER. \ignore{Rather, the single ring saturates at a lower injection
%rate, closer to the bufferless mesh design, CHIPPER. As network size scales to 8x8,
%HiRD performs significantly better relative to the meshes, because the
%hierarchy reduces the cross-chip latency while preserving bisection bandwidth.}
%
%2. Compared to a flattened butterfly design, we observe that HiRD performs
%competitively with a flattened butterfly in a 4x4 network, but consumes lower
%router power. In an 8x8 network, HiRD does not scale as well as a flattened
%butterfly network and performs 11\% worse than a flattened butterfly network
%but consumes 59\% less power than the flattened butterfly design. 
%
%
%\ignore{
%We compared our mechanism against a buffered mesh design with buffer bypassing.
%We configure the buffered mesh to have 4 VCs per port with 8 buffers per VC. 
%We also compare our mechanism against CHIPPER~\cite{chipper}, 
%a bufferless mesh network. We use 128-bit links on both design. 
%\ignore{Additionally,
%we compared our mechanism against a flattened butterfly design topology~\cite{flattened_bfly} with
%4 VCs per output port, 8 buffered per VC and 64-bit links.} We observe that HiRD performs very
%closely to the buffered mesh design in 4x4, saturating at nearly the same
%injection rate but maintaining a slightly lower network latency at high load.
%The buffered hierarchical ring saturates at a similar point to HiRD and the
%buffered mesh, but maintains a slightly lower average latency because it avoids
%transfer deflections. In contrast to these high-capacity designs, the single
%ring saturates at a lower injection rate, closer to the bufferless mesh design,
%CHIPPER. As network size scales to 8x8, HiRD performs significantly better
%relative to the meshes, because the hierarchy reduces the cross-chip latency
%while preserving bisection bandwidth.
%
%\begin{figure}[h!]
%\centering
%%\vspace{-.2in}
%\includegraphics[width=5in]{plots/WS_power8.pdf}
%%\vspace{-.2in}
%\caption{Weighted speedup (Y) vs. power (X) for 8x8 networks.}
%%\vspace{-.1in}
%\label{fig:WS_power8}
%\end{figure}
%
%Figure~\ref{fig:WS_power8} shows the energy efficiency comparison for an 8x8
%network. We only show HiRD with 8 bridge configuration, but varying the number
%of bridge router yield similar observation as a 4x4 network. The result shows that
%HiRD is more energy efficient compared to every other ring designs, and also 
%provides better energy efficiency compared to most other network designs. While
%CHIPPER consume roughly 33\% less power compared to HiRD. The performance of
%HiRD is 5.87\% better than that of CHIPPER. In addition, comparing to the best
%performing flattened butterfly network, HiRD performs roughly 10.67\% worse,
%but consumes 60\% less power.
%
%Overall, we conclude that HiRD either outperforms or is on-par with
%other baseline routers with respect to performance and energy
%efficiency. In cases where its efficiency is close to other designs,
%the other designs require more complex routers, and HiRD's design
%simplicity remains an advantage, because it reduces both
%design/validation effort and router die area.
%
%}
%
%
%
%
%
%\subsection{Alternative Topologies: Mesh, Ring, and Others}
%\label{sec:eval-topos}
%
%
%\begin{figure}
%\centering
%\includegraphics[width=3in]{plots/eval_main_compact.pdf}
%\caption{\small Evaluation against a variety of baseline designs.}
%\label{fig:eval-topo}
%\end{figure}
%
%\begin{figure}[h!]
%\centering
%\includegraphics[width=3.5in]{plots/WS_power.pdf}
%\caption{Weighted speedup (Y) vs. power (X) for 4x4 networks.}
%\label{fig:WS_power}
%\end{figure}
%
%
%
%
%Fig.~\ref{fig:eval-topo} shows a comparison of HiRD against a single ring, a
%mesh with VC-buffered routers~\cite{principles} (4 VCs with 4 flits/VC), a
%bufferless mesh (CHIPPER~\cite{chipper}), a concentrated mesh, and the buffered
%hierarchical ring network~\cite{ravindran97}.
%%  \footnote{We also compare to a flattened
%%  butterfly~\cite{flattened_bfly} VC-buffered configuration, but only
%%  for 4x4 (as the routers become very large at 8x8): the FBFly
%%  topology yields 4.7\% better performance than the buffered mesh on
%%  our workloads at 7.1\% less power. However, HiRD's substantial power
%%  and energy-efficiency advantage remains (68\% better energy
%%  efficiency). For uniformity, we omit FBFly from our main results
%%  plots.}
%As before, we show weighted speedup (application
%performance) and total network power, both normalized per node, as
%well as energy efficiency (performance per watt). Several main
%conclusions can be drawn:
%
%\noindent 1.  Overall, HiRD is competitive in performance with all baselines.
%In particular, it performs within 0.1\% (2\%) performance compared to the
%buffered mesh in 4x4 (8x8) networks. Though it is outperformed slightly by a
%concentrated mesh (in 4x4), both of these baseline designs require more complex
%mesh routers.
%
%\noindent 2. HiRD reduces network power significantly relative to the
%4x4 and 8x8 mesh routers, and is nearly on-par with CHIPPER in
%a 4x4 network. In the larger configuration, relative to the
%mesh routers, HiRD reduces static power (because mesh router crossbars
%are eliminated) but slightly increases link power (both because of
%ring deflections and because the path between two nodes may not be as
%direct as in a mesh).
%
%\noindent 3. Overall, HiRD is the most energy-efficient network design
%in 4x4 networks,  and is within 35\% of CHIPPER (the
%most energy-efficient baseline) in 8x8. However, while CHIPPER is more
%energy efficient because it consumes low power, as observed in previous 
%work~\cite{chipper}, CHIPPER performs 5\% worse and 19.6\% worse when
%the workloads are medium and high intensity, respectively.
%
%
%Fig.~\ref{fig:WS_power} highlights the energy-efficiency comparison by
%showing weighted speedup (Y axis) against power (X axis) for all
%evaluated networks in 4x4. HiRD is shown at three data points with the
%three bridge-router configurations (described in
%\S\ref{sec:bridge_router}). The top-left is the ideal corner (high
%performance, low power). As the results show, all three configurations
%of HiRD are more energy efficient than the evaluated baseline designs
%at this network size.
%
%Overall, we conclude that HiRD either outperforms or is on-par with
%other baseline routers with respect to performance and energy
%efficiency. In cases where its efficiency is close to other designs,
%the other designs require more complex mesh routers, and HiRD's design
%simplicity remains an advantage, because it reduces both
%design/validation effort and router die area.
%
%


==> secs/livelock_new.tex <==
\section{Guaranteed Delivery:  \qquad  \qquad  \qquad  \qquad \qquad \qquad Correctness in Hierarchical Ring Interconnects}
\label{sec:livelock}
\label{sec:guarantees}

In order for the system to operate correctly, the interconnect must guarantee
that every flit is eventually delivered to its destination. HiRD ensures
correct operation through two mechanisms that provide two guarantees: the
\emph{injection guarantee} and the \emph{transfer guarantee}. The injection
guarantee ensures that any flit waiting to inject into a ring will eventually
be able to enter that ring. The transfer guarantee ensures that any flit
waiting to enter a bridge router's transfer queue will eventually be granted a
slot in that queue. 

%These guarantees must be provided explicitly because HiRD's
%deflection-based ring transfers might otherwise cause a flit to remain in the
%network for an unbounded time. Together, the mechanisms that we introduce to
%ensure these two properties provide an end-to-end guarantee that all flits will
%be delivered.


To understand the need for each guarantee, let us consider an example, shown in
Figure~\ref{fig:guarantee-motivation}. A flit is enqueued for network injection
at node N1 on the leftmost local ring. This flit is destined for node N2 on the
rightmost local ring; hence, it must traverse the leftmost local ring, then the
global ring in the center of the figure, followed by the rightmost local ring.
The flit transfers rings twice, at the two bridge routers B1 and B2 shown in
the figure. The figure also indicates the six points (labeled as \mycirc{1} to
\mycirc{6}) at which the flit moves from a queue to a ring or vice-versa: the
flit first enters N1's injection queue, transfers to the leftmost local ring
\mycirc{1}, the bridge router B1 \mycirc{2}, the global ring \mycirc{3}, the
bridge router B2 \mycirc{4}, the rightmost local ring \mycirc{5}, and finally
the destination node N2 \mycirc{6}.


\begin{figure}[h]
\centering
\vspace{-0.2in}
\includegraphics[width=2.8in]{figs/guarantee-motivation.pdf}
\caption{\footnotesize \bf The need for the injection and transfer guarantees:
  contention experienced by a flit during its journey.}
\label{fig:guarantee-motivation}
\vspace{-0.15in}
\end{figure}

In the worst case, when the network is heavily contended, the flit
could wait for an unbounded amount of time at \mycirc{1} to
\mycirc{5}. First, recall that to enter any ring, a flit must wait for an empty
slot on that ring (because the traffic on the ring continues along the
ring once it has entered, and thus has higher priority than any new
traffic). Because of this, the flit traveling from node N1 to N2 could
wait for an arbitrarily long time at \mycirc{1}, \mycirc{3}, and \mycirc{5}  if no other
mechanism intercedes. This first problem is one of \emph{injection
  starvation}, and we address it with the \emph{injection guarantee}
mechanism described below. Second, recall that a flit that needs to
transfer from one ring to another via a bridge router enters that
bridge router's queue, but if the bridge router's queue is full, then
the transferring flit must make another trip around its current ring
and try again when it next encounters a bridge router. Because of this
rule, the flit traveling from N1 to N2 could be \emph{deflected} an
arbitrarily large number of times at \mycirc{2} and \mycirc{4} (at entry to
bridge routers B1 and B2) if no other mechanism intercedes. This
second problem is one of \emph{transfer starvation}, and we address it
with the \emph{transfer guarantee} mechanism described below.


\emph{Our goal} in this section is to demonstrate that HiRD provides both the
injection guarantee (\S\ref{sec:guarantee-injection}) and the transfer guarantee
(\S\ref{sec:guarantee-transfer}) mechanisms. We show correctness
in \S\ref{sec:guarantee-correctness}, and quantitatively evaluate both
mechanisms in \S\ref{sec:eval-guarantees} and in~\cite{hird-safari-tr}.

\subsection{Preventing Injection Starvation: Injection Guarantee}
\label{sec:guarantee-injection}

The \emph{injection guarantee} ensures that every router on a ring can
eventually inject a flit. This guarantee is provided by a very simple
throttling-based mechanism: when any node is starved (cannot inject a flit)
past a threshold number of cycles, it asserts a signal to a global controller,
which then throttles injection from every other node. No new traffic will enter
the network while this throttling state is active. All existing flits in the
network will eventually drain, and the starved node will be able to finally
inject its new flit. At that time, the starved node de-asserts its throttling
request signal to the global controller, and the global controller subsequently
allows all other nodes to resume normal operation. 
%While we will more formally
%argue correctness below, this injection guarantee mechanism is correct simply
%because the throttling remains active until the starved node's flit is
%injected; in the most extreme case, all flits in the network will drain, and
%the starved node will be able to inject (in most cases, the problem resolves
%before all flits drain). Thus, HiRD provides an injection guarantee.


Note that this injection guarantee can be implemented in a hierarchical manner
to improve scalability. In the hierarchical implementation, each individual
local ring in the network monitors only its own injection and throttles
injection locally if any node in it is starved. After a threshold number of
cycles.\footnote{In our evaluation, we set this threshold to be 100 cycles.} if
any node in the ring still cannot inject, the bridge routers connected to that
ring start sending throttling signals to any other ring in the next level of
the ring hierarchy they are connected to. In the worst case, every local ring
stops accepting flits and all the flits in the network drain and eliminate any
potential livelock or deadlock. Designing the delivery guarantee this way 
requires two wires in each ring and small design overhead at
the bridge router to propagate the throttling signal across hierarchy levels. In our
evaluation, we faithfully model this hierarchical design.


\ignore{
Note that a global throttling-based approach is not necessarily the
most optimal method to ensure a flit has an empty slot to enter the
network. In the best case, exactly one other new injection could be
throttled in order to create one empty slot into which the starved
node could inject its flit (i.e., a one-for-one trade in new flit
injections). \emph{However}, such a scheme would require significant
global coordination and run-time planning: some central authority
would have to find an empty slot in the network (in the worst case,
when the network is completely full everywhere, wait for some flit to
be delivered and removed from its ring) and explicitly mark that slot
as reserved for the starved node. In contrast, as long as starvation
events are \emph{rare}, it is much simpler to temporarily inhibit
injection from all nodes until the problem is (quickly) addressed as
space is freed. In fact, in our evaluations of real application works,
we observe that injection starvation events are exceedingly rare and
hence their bandwidth efficiency has little impact on overall
throughput. Our quantitative evaluation of the injection guarantee
mechanism in \S\ref{sec:eval-guarantees} will show that sufficient
throughput remains even in a worst-case synthetic traffic pattern for
injection starvation.
}

\subsection{Ensuring Ring Transfers: Transfer Guarantee}
\label{sec:guarantee-transfer}

The \emph{transfer guarantee} ensures that any flit waiting to transfer from
its current ring to another ring via a bridge router will eventually be able to
enter that bridge router's queue. Such a guarantee is non-trivial because the
bridge router's queue is finite, and when the destination ring is congested, a
slot may become available in the queue only infrequently. In the worst case, a
flit in one ring may circulate indefinitely, finding a bridge router to its
destination ring with a completely full queue each time it arrives at the
bridge router. The transfer guarantee ensures that any such circulating flit
will eventually be granted an open slot in the bridge router's transfer queue.
Note in particular that this guarantee is \emph{separate from} the injection
guarantee: while the injection guarantee ensures that the bridge router will be
able to inject flits from its transfer queue into the destination ring (and
hence, have open slots in its transfer queue eventually), these open transfer
slots may not be distributed \emph{fairly} to flits circulating on a ring
waiting to transfer through the bridge router. In other words, some flit may
always be ``unlucky'' and never enter the bridge router if slots open at the
wrong time. The transfer guarantee addresses this problem.

In order to ensure that any flit waiting to transfer out of a ring
eventually enters its required bridge router, each bridge router
\emph{observes a particular slot on its source ring} and monitors for
flits that are ``stuck'' for more than a threshold number of
retries. (To observe one ``slot,'' the bridge router simply examines
the flit in its ring pipeline register once every N cycles, where N is
the latency for a flit to travel around the ring once.) If any flit
circulates in its ring more than this threshold number of times, the
bridge router reserves the next open available entry in its transfer queue for
this flit (in other words, it will refuse to accept other flits for
transfer until the ``stuck'' flit enters the queue). Because of the
injection guarantee, the head of the transfer queue must inject into
the destination ring eventually, hence an entry must become available eventually,
and the stuck flit will then take the entry in the transfer queue the
next time it arrives at the bridge router. Finally, the slot which the
bridge router observes rotates around its source ring: whenever the
bridge router observes a slot the second time, if the flit that
occupied the slot on first observation is no longer present (i.e.,
successfully transferred out of the ring or ejected at its
destination), then the bridge router begins to observe the \emph{next}
slot (the slot that arrives in the next cycle). In this way, every
slot in the ring is observed eventually, and any stuck flit will thus
eventually be granted a transfer.

\subsection{Putting it Together: Guaranteed Delivery}
\label{sec:guarantee-correctness}

%We now formally prove the end-to-end delivery guarantee for any flit
%in the network given the injection and transfer guarantees described
%above.


\linespread{1}
\begin{table*}
\vspace{-0.25in}
\centering
\footnotesize{
\begin{tabular}{|l||p{14.8cm}|}
\hline
\textbf{Parameter} & \textbf{Setting} \\
\hline
\hline
System topology & CPU core and shared cache slice at every node \\
\hline
Core model & Out-of-order, 128-entry ROB, \\16 MSHRs (maximum simultaneous outstanding requests) \\
\hline
Private L1 cache & 64 KB, 4-way associative, 32-byte block size \\
\hline
Shared L2 cache & Perfect (always hits) to stress the network and
penalize our reduced-capacity deflection-based design; cache-block-interleaved
%\footnote{We also evaluated our system with a realistic memory and the
%result shows similar trend, with slightly smaller performance and power
%efficiency gap.}
%mapping
 \\
\hline
Cache coherence & Directory-based protocol (based on SGI
Origin~\cite{laudon97}), directory entries co-located with
shared cache blocks \\
\hline
Simulation length & 5M-instruction warm-up, 25M-instruction active execution per node
%\footnote{We verified with a
%smaller set of workloads that the trends observed with 25M instructions are representative of those observed with longer runs.
%Applications continue running even after 25M instructions until every application finishes in order to make sure cores are fully utilized. }
~\cite{casebufferless,chipper,hat-sbac-pad,minbd} \\
\hline
\end{tabular}
}
\caption{\footnotesize \bf Simulation and system configuration parameters.}
\vspace{-0.15in}
\label{table:sysparams}
\end{table*}

\begin{table*}
\centering
\footnotesize{
\begin{tabular}{|l|l|p{12.5cm}|}
\hline
Parameter & Network & Setting \\
\hline
\hline
\multirow{4}{*}{Interconnect Links} & Single Ring & Bidirectional, \textbf{4x4:} 64-bit and 128-bit width, \textbf{8x8:} 128-bit and 256-bit width \\
\cline{2-3}
& Buffered HRing & Bidirectional, \textbf{4x4:} 3-cycle per-hop latency (link+router); 64-bit local and 128-bit global rings, \textbf{8x8:} three-level hierarchy, 4x4 parameters, with second-level rings connected by a 256-bit third-level ring \\
\cline{2-3}
& HiRD & \textbf{4x4:} 2-cycle (local), 3-cycle (global) per-hop
latency (link+router); 64-bit local ring, 128-bit global ring; \textbf{8x8:} 4x4
parameters, with second-level rings connected by a 256-bit third-level
ring \\
\hline 
\multirow{6}{*}{Router} & Single Ring & 1-cycle per-hop latency (as in~\cite{kim09nocarc}) \\
\cline{2-3}
& Buffered HRing & Node (NIC) and bridge (IRI) routers based
on~\cite{ravindran97}; 4-flit in-ring and transfer
FIFOs. Bidirectional links of dual-flit width (for fair comparison
with our design). Bubble flow control~\cite{bubbleflow} for deadlock
freedom. \\
\cline{2-3}
& HiRD & Local-to-global buffer depth of 1, global-to-local buffer depth of 4 \\
\hline
\end{tabular}
}
\caption{\footnotesize \bf Network parameters.}
\vspace{-0.25in}
\label{table:topoparams}
\end{table*}

\linespread{0.85}


%TODO: Can delete this?
Before we prove the correctness of these mechanisms in detail, it is helpful to
summarize the basic operation of the network once more. A flit can inject into
a ring whenever a free slot is present in the ring at the injecting router
(except when the injecting router is throttled by the injection guarantee
mechanism). A flit can eject at its destination whenever it arrives, and
destinations always consume flits as soon as they arrive (which is ensured
despite finite reassembly buffers using the Retransmit-Once mechanism~\cite{chipper}, as
already described in \S\ref{sec:mech-node-router}). A flit transfers between
rings via a transfer queue in a bridge router, first leaving its source ring to
wait in the queue and then injecting into its destination ring when at the head
of the queue, and can enter a transfer queue whenever there is a free entry in
that transfer queue (except when the entry is reserved for another flit by the
transfer guarantee mechanism). Finally, when two flits at opposite ends of a
bridge router each desire to to transfer through the bridge router, the
\emph{Swap Rule} allows these flits to exchange places directly, bypassing the
queues (and ensuring forward progress).

Our proof is structured as follows: we first argue that if no new flits enter
the network, then the network will drain in finite time. The injection
guarantee ensures that any flit can enter the network. Then, using the
injection guarantee, transfer guarantee, the swap rule, and the fact that the
network is hierarchical, any flit in the network can eventually reach any ring
in the network (and hence, its final destination ring). Because all flits in a
ring continue to circulate that ring, and any node on a ring must consume any
flits that are destined for that node, final delivery is ensured once a flit
reaches its final destination ring.

\noindent\textbf{Network drains in finite time:} Assume no new flits enter the
network (for now). A flit could only be stuck in the network indefinitely if
transferring flits create a cyclic dependence between completely full rings.
Otherwise, if there are no dependence cycles, then if one ring is full and
cannot accept new flits because other rings will not accept \emph{its} flits,
then eventually there must be some ring which depends on no other ring (e.g., a
local ring with all locally-destined flits), and this ring will drain first,
followed by the others feeding into it. However, because the network is
hierarchical (i.e., a tree), the only cyclic dependences possible are between
rings that are immediate parent and child (e.g., global ring and local ring, in
a two-level hierarchy). The \emph{Swap Rule} ensures that when a parent and
child ring are each full of flits that require transfer to the other ring, then
transfer is always possible, and forward progress will be ensured. Note in
particular that we do not require the injection or transfer guarantee for the
network to drain. Only the \emph{Swap Rule} is necessary to ensure that no deadlock
will occur. \ignore{As long as flits continue to drain, no flit waiting in a
transfer queue can be starved from injecting into its destination ring for more
than a finite amount of time.}


\noindent\textbf{Any node can inject:} Now that we have shown that the network
will drain if no new flits are injected, it is easy to see that the injection
guarantee ensures that any node can eventually inject a flit: if any node is
starved, then all nodes are throttled, no new flit enters the network, and the
network must eventually drain (as we just showed), at which point the starved
node will encounter a completely empty network into which to inject its flit.
(It likely will be able to inject before the network is completely empty, but
in the worst case, the guarantee is ensured in this way.)

\noindent\textbf{All flits can transfer rings and reach their destination
rings:} With the injection guarantee in place, the transfer guarantee can be
shown to provide its stated guarantee as follows: because of the injection
guarantee, a transfer queue in a bridge router will always inject its head flit
in finite time, hence will have an open entry to accept a new transferring flit
in finite time. All that is necessary to ensure that \emph{all} transferring
flits eventually succeed in their transfers is that \emph{any} flit stuck for
long enough gets an available entry in the transfer queue. The transfer
guarantee does exactly this by observing ring slots in sequence and reserving a
transfer queue entry when a flit becomes stuck in a ring. Because the mechanism
will eventually observe every slot in the ring, all flits will be allowed to make their
transfers eventually. Hence, all flits can continue to transfer rings until
reaching their destination rings (and thus, their final destinations).



\subsection{Hardware Cost}

Our injection and transfer guarantee mechanisms have low hardware overhead. To implement the
injection guarantee, one counter is required for each injection point.
This counter tracks how many cycles have elapsed while injection is starved,
and is reset whenever a flit is successfully injected. Routers communicate with
the throttling arbitration logic with only two wires, one to signal blocked
injection and one control line that throttles the router. The wiring is done
hierarchically instead of globally to minimize the wiring cost (\S\ref{sec:guarantee-injection}). Because the
correctness of the algorithm does not depend on the delay of these wires, and
the injection guarantee mechanism is activated only rarely (in fact, \emph{never} for
our evaluated realistic workloads), the signaling and central coordinator need not be
optimized for speed. To provide the transfer guarantee, each bridge router
implements ``observer'' functionality for each of the two rings it sits on, and
the observer consists only of three small counters (to track the current
timeslot being observed, the current timeslot at the ring pipeline register in
this router, and the number of times the observed flit has circled the ring)
and a small amount of control logic.  Importantly, note that neither mechanism
impacts the router critical path nor affects the router datapath (which
dominates energy and area).


==> secs/motivation.tex <==
\section{Motivation}
\label{sec:motivation}

In this section, we first show how ring routers can be very simple, but not
scalable. We then describe past work in hierarchical rings and show how a
previous design obtained performance scalability with rings, but required
reintroducing in-ring flow control and buffering, thereby obviating the primary
benefits of rings.  These two observations -- rings are simple but do not
scale, and a hierarchy of rings scales but increases complexity --
motivate our \emph{simple} hierarchical ring interconnect, HiRD.



%In this section, we first argue that (i) ring routers can be very
%simple, compared to mesh routers, but that (ii) meshes are more
%scalable than single rings. We then describe past work in hierarchical
%rings and show how a previous design obtained performance scalability
%with rings but required in-ring flow control and buffering, which led
%to complicated ring routers. These two observations -- the scalability
%of rings given hierarchy, but the complexity of prior approaches to
%hierarchical rings -- motivate our \emph{simple} hierarchical ring
%interconnect, HiRD.

\subsection{Simplicity in Ring-Based Interconnects}

Ring interconnects are attractive in current small-to-medium-scale
commercial CMPs because ring routers (ring stops) are simple, which
leads to smaller die area and energy overhead. In its simplest form, a
ring router needs to perform only two functions: injecting new traffic
into the ring, and removing traffic from the ring when it has arrived
at its destination. Figure~\ref{fig:ring-router} a) depicts the router
datapath and control logic (at a high level) necessary to implement
this functionality. For every incoming \emph{flit} (unit of data
transfer as wide as one link), the router only needs to determine
whether the flit stays on the ring or exits at this node. Then, if a
flit is waiting to inject, the router checks whether a flit is already
present on the ring in this timeslot, and if not, injects the new flit
using the in-ring MUX.

\begin{figure}[h]
\centering
\includegraphics[width=3.4in]{figs/ring-router}
%\caption{\small a) A ring router. b) Buffered hierarchical ring
%  detail, as proposed in prior work: one
%  \emph{bridge router} which connects two rings.}
\caption{\small a) A ring router. b) Buffered hierarchical ring detail, as proposed in prior
  work~\protect\cite{ravindran97}: one \emph{bridge router} which connects two
  rings.}
\label{fig:ring-router}
\end{figure}

Rings achieve very good energy efficiency at low-to-medium core
counts~\cite{kim09nocarc}; However, the simplicity advantage of a ring-based
network, rings have a fundamental \emph{scalability} limit: a ring stops
scaling at fewer nodes because its bisection bandwidth is \emph{constant}
(proportional only to link width) and the average hop count (which translates
to latency for a packet) increases linearly with the number of nodes. (In the
worst case for a bidirectional ring, a packet visits half the network on its
way to its destination, and a quarter on average.)

%
%\begin{figure}
%\centering
%\subfloat[\small A ring router.]{
%\includegraphics[width=1.2in]{figs/ring-router.pdf}
%\label{fig:ring-router}
%}
%\hspace{0.1in}
%\subfloat[\small A mesh router.]{
%\includegraphics[width=1.8in]{figs/mesh-router.pdf}
%\label{fig:mesh-router}
%}
%\end{figure}

%In contrast, mesh-based interconnects, and other interconnects in
%which routers have higher \emph{radix} (more connections to
%neighboring routers), require more complex
%routers. Fig.~\ref{fig:mesh-router} depicts the router datapath and
%control logic necessary to implement a standard input-buffered (VC)
%mesh router~\cite{principles}. For every incoming flit, the router
%stores the flit in a buffer, and also computes what the flit's next
%hop should be (\emph{Route Computation}. This computation determines
%\emph{which} output port the flit must take. Once this is known, the
%flit can arbitrate for a downstream buffer (\emph{VC Arbitration}) and
%the datapath to the router output (\emph{Switch Alloc}) before
%traversing the crossbar. All of these steps add energy and die area
%overhead that is not present in the simple ring-based
%router. Additionally, the design and validation effort required to
%correctly implement such a router is significantly higher than that
%for a simple ring router.


%\subsection{Scalability in Mesh-Based Interconnects}
%
%Despite the simplicity advantage of a ring-based network, rings have a
%fundamental \emph{scalability} limit: as compared to a mesh, a ring
%stops scaling at fewer nodes because its bisection bandwidth is
%\emph{constant} (proportional only to link width) and the average hop
%count (which translates to latency for a packet) increases linearly
%with the number of nodes. (Intuitively, a packet visits half the
%network on its way to the destination, in the worst case, and a
%quarter in the average case, for a bidirectional ring.) In contrast, a
%mesh has bisection bandwidth proportional to one dimension of the
%layout (e.g., the square-root of the node count for a 2D mesh) and
%also has an average hop count that scales only with one dimension. The
%higher radix, and thus higher connectivity, of the mesh allows for
%more path diversity and lower hop counts which increases performance.
%
%To demonstrate this problem quantitatively, we show application
%performance averaged over a representative set of network-intensive
%workloads on (i) a single ring network and (ii) a conventional 2D-mesh
%buffered interconnect (details in \S\ref{sec:meth}). As the
%plot shows, although the single ring is able to match the mesh's
%performance at the 16-node design point, it degrades when node count
%increases to 64. Note that in this case, the ring's bisection
%bandwidth is kept equivalent to the mesh, so the performance
%degradation is solely due to higher hop count; considerations of
%practical ring width might reduce performance further.
%
%\begin{figure}
%\centering
%\includegraphics[width=2in]{plots/motivation-scale-perf.pdf}
%\caption{\small Performance as mesh and ring networks to 64 nodes.}
%\label{fig:motivation-scale-perf}
%\end{figure}

\subsection{Hierarchical Rings for Scalability}

%So far, we have seen that (i) ring routers are very simple in
%comparison to mesh routers, but that (ii) a mesh offers better
%performance scalability at high node counts. Ideally, we would like a
%simple yet scalable interconnect.

Fortunately, past work has observed that \emph{hierarchy} allows for
additional scalability in many interconnects: in ring-based
designs~\cite{ravindran97,xiangdong95,hr-model,ravindran98,numachine},
with hierarchical buses~\cite{udipi10}, and with hierarchical
meshes~\cite{das09}.  The state-of-the-art hierarchical ring
design~\cite{ravindran97} in particular reports promising results by
combining local rings with one or more levels of higher-level rings,
which we refer to as global rings, that connect lower level rings
together.  Rings of different levels are joined by Inter-Ring
Interfaces (IRIs), which we call ``bridge routers'' in this
work. Figure~\ref{fig:ring-router} b) graphically depicts the details of
one bridge router in the previously proposed buffered hierarchical
ring network.

%GLOH
%{\color{red} Gabe: I'm not entirely sure ``global'' is the right term we
%want to use for the higher-level rings... it strikes me as inaccurate
%and possibly midleading/confusing.  In a three-level hierarchy, the
%second-level is certainly not ``global'', and even the top-level one
%doesn't seem entirely ``global'' to me... it's analogous to calling
%the root of a tree the ``global'' node (which while in some sense may
%be true, it just isn't immediately intuitive to me).}


Unfortunately, connecting multiple rings via bridge routers introduces
a new problem.  Recall that injecting new traffic into a ring requires
an open slot in that ring. If the ring is completely full with flits
(i.e., a router attempting to inject a new flit must instead pass
through a flit already on the ring every cycle), then no new traffic
will be injected. But, a bridge router must inject transferring flits
into those flits' destination ring in exactly the same manner as if
they were newly entering the network. If the ring on one end of the
bridge router is completely full (cannot accept any new flits), and
the transfer FIFO into that ring is also full, then any other flit
requiring a transfer must \emph{block} its current ring. In other
words, ring transfers create new dependences between adjacent rings,
which creates the need for end-to-end flow control. This flow control
forces every node router (ring stop) to have an in-ring FIFO and flow
control logic, which increases energy and die area overhead and
significantly reduces the appeal of a simple ring-based
design. Table~\ref{table:power_area} compares the power consumption
for a previously proposed hierarchical ring design (Buffered HRing)
and a bufferless hierarchical ring design on a system with 16 nodes
using DSENT 0.91~\cite{dsent} and a 45nm technology commercial design
library. In the examined idealized bufferless design, each ring has no
in-ring buffers, but there are buffers between the hierarchy
levels. When a packet needs a buffer that is full, it gets deflected
and circles its local ring to try again. Clearly, eliminating in-ring
buffers in a hierarchical ring network can reduce power and area
significantly.

%%% ONUR: Is the above bufferless design the same as HiRD, or is it an
%%% "idealized" design with no buffers but also no mechanisms for
%%% livelock prevention.

%%% ONUR: See what I added above: "In the examined idealized
%%% bufferless design, each ring has no in-ring buffers, but there are
%%% buffers between the hierarchy levels." Is this correct? There
%%% needs to be some detail on the bufferless network.
%% Rachata: That is correct. There is no in-ring buffers but there are
%% buffers between hierarchy levels.

\begin{table}[h!]
\centering
\footnotesize{
\vspace{-0.1in}
\begin{tabular}{|p{2.2cm}||p{2.2cm}|p{2.2cm}|}
\hline
Metric & Buffered HRing & Bufferless HRing \\
\hline
\hline
Normalized power & 1 & 0.535 \\
\hline
Normalized area & 1 & 0.495 \\
\hline
\end{tabular}
}
%\vspace{-0.1in}
\caption{\small Power and area comparison (16-node network).}
\label{table:power_area}
\vspace{-0.15in}
\end{table}

However, simply removing in-ring buffers can introduce livelock, as a
deflected packet may circle its local ring indefinitely. Our goal in
this work is to introduce a hierarchical ring design that maintains
simplicity and low cost, while ensuring livelock and deadlock freedom
for packets.

%In this work, we introduce HiRD, which solves this
%problem in a low-cost way.

%TODO: rausavar: Add a comparison between a buffered hring and a bufferless hring


% TODO: cfallin: system that uses drops in this situation? Cite it
% here?

% ---- old motivation below -----

\ignore{
\subsection{Energy Efficiency in Ring-Based Interconnects}
\label{sec:motivation-energy}

Rings achieve very good energy efficiency at low-to-medium core
counts~\cite{kim09nocarc}, or when network load is low enough that the
ring does not become a bottleneck. The routing logic for a router in a
single-ring system needs to handle only two tasks: injecting traffic
into a ring when there is space, and ejecting traffic that is
addressed to the current router. Most energy consumed in the
interconnect is thus due to link traversal -- in other words, the
router energy is minimal because the routers are very simple. The
simplicity, and thus low design/validation cost, are further
advantages.

In order to understand the behavior of rings relative to meshes more
concretely, let us examine data from application workloads on a
medium-sized (16 node) CMP. In Figure~\ref{fig:motivation-energy}, we
show application performance and average network power for a set of 60
multiprogrammed (SPEC CPU2006~\cite{spec}) workloads on a 16-node
system with either a single ring or a conventional 2D-mesh (4x4)
buffered interconnect. (See~\S\ref{sec:meth} for methodology and
workload categorization.) The workloads are split into two categories
based on the constituent applications' cache miss rates, and thus
network-injection rates: \textbf{L}, or ``low-intensity'', which have
a low injection rate (0.03 flits/node/cycle on average),
and \textbf{H}, or ``high-intensity,'' which stress the network with
higher injection rates (0.46 flits/node/cycle average injection rate).
%%% ONUR-11-20: Can you be more concrete about H and L categories. (2-3 word description of each is possible?) -- I fixed this by adding ``workload categorization'' above.

%%% cfallin - also added injection rates here.

First, as the data in the figure demonstrate, for a medium-sized
(16-core) system configuration, the single ring slightly exceeds the
performance of a 2D mesh at low load, because the smaller router
latency (1 cycle rather than 2 cycles) enables higher performance. In
fact, the single ring maintains competitive performance with a mesh up
through medium-intensity workloads, as we show
in \S\ref{sec:eval-perf}. However, with the set of
high-network-intensity workloads, in which performance depends more
heavily on NoC throughput, performance degrades 27.1\% relative to the
mesh. Hence, although the network begins to hit scaling limits when
stressed, it performs very well at low load.

%%% ONUR-11-20: Is it true that the NoC is the system bottleneck with high intensity workloads?

%%% cfallin: ``in which performance depends more heavily on NoC
%%% throughput'' now. True, it may not be the only system bottleneck
%%% in general (though here it is since we run with a perfect L2).

The true advantage of the ring design is seen by examining total
interconnect power. The average network power shown in the figure
indicates that the ring consumes 76.3\% less power on average with
workloads that have low network intensity, and 26.7\% less power at
high network intensity. Hence, even at saturation, the ring consumes
less power on average. This reduction is due to the much simpler ring
router design, compared to the buffered mesh: while the mesh router
requires a large, power-hungry crossbar and input buffers, the ring
router can consist only of several pipeline registers and MUXes (as we
describe in more detail later). Furthermore, because power reduction
(as a fraction of the baseline mesh) is greater than the performance
degradation even at the highest load, the ring is the more
energy-efficient design when only network energy is considered.

%%% ONUR-11-20: can you very briefly justify the reason for reduced power?
%%% cfallin--done.
%%% ONUR-11-20: Can you change y-axis labels in Figs 1-2 from ``power (mW)'' to ``Network Power (mW)''
%%% cfallin--done.

%%% ONUR-11-20: Also in Fig 1-2: ``buffered-mesh'' --> ``Buffered-mesh''
%%% cfallin--done.

\begin{figure*}[h]
\centering
\includegraphics[width=5in,height=1in]{plots/motivation-energy.pdf}
\caption{\small Performance and average network power for 16 nodes, in mesh
  and ring interconnects.}
\label{fig:motivation-energy}
\end{figure*}

\subsection{Scaling Limits of a Single-Ring Interconnect}
\label{sec:motivation-scaling}

Unfortunately, as network size increases, ring-based designs scale
poorly, relative to mesh-based designs. This is fundamentally due to
\emph{ring contention}: a ring saturates more quickly as load
increases because all traffic passes through every node between the
source and destination. This traffic then prevents any node along the
path from injecting additional traffic. In contrast, a mesh is able to
handle higher load per network node, because it has more links per
node and more path diversity.\ignore{a greater number of possible
  paths for a given journey.}

\begin{figure*}[h]
\centering
\includegraphics[width=5in,height=1in]{plots/motivation-scale.pdf}
\caption{\small Performance and power as mesh and ring networks scale from 16
  to 64 nodes.}
\label{fig:motivation-scaling}
\end{figure*}

%%% ONUR-11-20: What are ``medium-network-intensity'' workloads? These are all defined clearly in methodology, right? -- I fixed this by adding ``workload categorization'' above.
We demonstrate the scaling limits of a single-ring design in
Figure~\ref{fig:motivation-scaling}. The figure shows average
performance and network energy for a set of medium-network-intensity
workloads (see \S\ref{sec:meth} for details) in both 16-core and
64-core configurations, for a single ring and a 2D-mesh buffered
interconnect. The ring width is increased so that the bisection
bandwidth is equivalent to the mesh design's bisection bandwidth at
both network sizes, for fair comparison. As the figure shows, in the
16-node configuration, the ring performs slightly better than the mesh
interconnect, again because of lower router latency. In contrast, when
the network size increases, the ring performs very poorly, with 34.2\%
lower performance than the mesh and 60.7\% higher network power (due
to increased link traversals).

We conclude that while a single-ring interconnect has excellent
energy-efficiency and satisfactory performance for low-to-medium
network load in medium-sized CMPs, performance and energy efficiency
drop significantly when the network load or network size
increases. Despite this shortcoming, the simplicity and efficiency of
a ring-based router are attractive.  \textbf{Our goal} in this paper
is to devise a new NoC design that achieves the energy-efficiency of a
ring router with the performance and scalability of mesh-based
designs.

%%% ONUR-11-20: You say ``low-to-medium network load'' above, but you
%%% did not show medium load explicitly in Fig 1 (true you have it in
%%% Fig 2). You can either say when you show low load workloads that
%%% medium load workloads show a similar trend. Or, you can include a
%%% new category in Fig 1, Medium-intensity. What do you think?

%%% cfallin--added forward reference to eval section above where
%%% Fig. 1 is discussed, and noted that medium-intensity workloads
%%% show a similar trend, with competitive performance on a single
%%% ring relative to buf-mesh.

}

